Improving Training-free Conditional Diffusion Model via Fisher Information

Training-free conditional diffusion models have received great attention in conditional image generation tasks. However, they require a computationally expensive conditional score estimator to let the intermediate results of each step in the reverse process toward the condition, which causes slow conditional generation. In this paper, we propose a novel Fisher information-based conditional diffusion (FICD) model to generate high-quality samples according to the condition. In particular, we further explore the conditional term from the perspective of Fisher information, where we show Fisher information can act as a weight to measure the informativeness of the condition in each generation step. According to this new perspective, we can control and gain more information along the conditional direction in the generation space. Thus, we propose the upper bound of the Fisher information to reformulate the conditional term, which increases the information gain and decreases the time cost. Experimental results also demonstrate that the proposed FICD can offer up to 2x speed-ups under the same sampling steps as most baselines. Meanwhile, FICD can improve the generation quality in various tasks compared to the baselines with a low computation cost.

==> sec/X_supply.tex <==
\clearpage
\setcounter{page}{1}
\section{Appendix}


\setcounter{equation}{0}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\setcounter{theorem}{0}
\renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
\section{PROOFS AND THEORETICAL ANALYSIS}
\subsection{PROOF OF THEOREM~\ref{th:convergent theory}}
\begin{theorem}
Given the sequence $\{\bm{x}_{T},\bm{x}_{T-1},...,\bm{x}_{t},...,\bm{x}_{1}\}$, where $t \in [T, 0)$ and $\bm{x}_{T}$ is the initial state of the reverse process, the $I(\bm{x}_{t})$ is convergent to the Cram$\acute{e}$r-Rao bound:
\begin{equation}
    \lim_{\Delta t \to 0} I(\bm{x}_{t + \Delta t}) = \frac{1}{1-\hat{\alpha}_{t}}.
    \label{eq:upper bound}
\end{equation}
\label{th:convergent theory_appendix}
\end{theorem}

\begin{proof}
The reverse process of the diffusion model could be formulated as:
\begin{equation}
    \bm{x}_{t-1} = \sqrt{\alpha_{t-1}}(\frac{\bm{x}_{t}-\sqrt{1-\alpha_{t}}\epsilon_{\theta}(\bm{x}_{t},t)}{\sqrt{\alpha_{t}}})+\sqrt{1-\alpha_{t-1}-\sigma^{2}_{t}\epsilon_{\theta}(\bm{x}_{t},t)}+\sigma_{t}\epsilon,
    \label{eq:ap_1}
\end{equation}
where $\alpha_{t-1}$, $\alpha_{t}$, $\sigma_{t}$ are the known parameters related to the noise schedule, $\epsilon_{\theta} \sim \mathcal{N}(0,1)$ is the pure Gaussian noise and $\epsilon_{\theta}(\ast,\ast)$ are the score function based on the parameter $\theta$. 

Then we organize Eq.~\ref{eq:ap_1} as:
\begin{equation}
\bm{x}_{t-1} = \frac{\sqrt{\alpha_{t-1}}}{\sqrt{\alpha_{t}}}\bm{x}_{t} + \bm{m}_{t}\epsilon_{\theta}(\bm{x}_{t},t)+\sigma_{t}\epsilon.
\label{eq:ap_2}
\end{equation}
where:
\begin{equation}
    \bm{m}_{t} = \sqrt{1-\alpha_{t-1}-\sigma^{2}_{t}} - \frac{\sqrt{\alpha_{t-1}}}{\sqrt{\alpha_{t}}}(\sqrt{1-\alpha_{t}}).
\end{equation}

We could build the time sequence related to the $\bm{x}_{t}$ based on Eq.~\ref{eq:ap_2} during $[t + \Delta t, t]$ as $S_{n} = \{\bm{x}_{t+\Delta t},...,\bm{x}_{t}\}$, where $n$ is sampling iterations. Then, recall the forward process:
\begin{equation}
    \bm{x}_{t} = \frac{\sqrt{a_{t}}}{\sqrt{a_{t-1}}}\bm{x}_{t-1} + (1-\frac{\alpha_{t}}{\alpha_{t-1}})\epsilon.
\end{equation}

Based on the property of the diffusion model, given the well pre-trained $\epsilon_{\theta}(\bm{x}_{t},t)$, we have:
\begin{equation}
    m_{t}\epsilon_{\theta}(\bm{x}_{t},t)+\sigma_{t}\epsilon \approx   (1-\frac{\alpha_{t}}{\alpha_{t-1}})\epsilon.
\end{equation}
By $j_{t} = \frac{\alpha_{t}}{\alpha_{t-1}}$, we further have:
\begin{equation}
    \bm{x}_{t-1} = \sqrt{j_{t}}\bm{x}_{t} + \sqrt{1-j_{t}}\epsilon.
    \label{eq:central sequance}
\end{equation}

In this way, the samples in $S_{n}$ satisfies the central limit theorem~\cite{InformationTheory}:
\begin{equation}
    \lim_{\Delta t \to 0} I(\bm{x}_{t + \Delta t}) = \frac{1}{1-\hat{\alpha}_{t}}.
\end{equation}
Thus, we finish the proof.
\end{proof}

\subsection{PROOF OF THEOREM~\ref{th:upperbound}}
\begin{theorem}
    For any $\bm{x}_{t}$ where $t \in [T, 0)$, the Fisher information $I(\bm{x}_{t})$ could be bounded as:
    \begin{equation}
        I(\bm{x}_{t}) < \lim_{\Delta t \to 0} I(\bm{x}_{t + \Delta t}) = \frac{1}{1-\hat{\alpha}_{t}}.
        \label{eq:upperbound}
    \end{equation}
    \label{th:upperbound}
\end{theorem}
\begin{proof}
    Based on the Theorem~\ref{th:convergent theory} and Eq.~\ref{eq:central sequance}, given the continuous time sequence $S_{n}$, for any time we all have the Cram$\acute{e}$r-Rao bound. Based on the property of the stochastic differential equation~\cite{sde}, during $[t + \Delta t, t]$, we could build the time sequence $S_{n}$ in each $t$. Therefore, in each $t$, it always exists the Cram$\acute{e}$r-Rao bound and thus we could use the Cram$\acute{e}$r-Rao bound as the estimate of $I(\bm{x}_{t})$. Then, with the decreasing of $t$, $\hat{a}_{t}$ will decrease. For $t + \Delta t > t$, we all have $I(\bm{x}_{t}) < \lim_{\Delta t \to 0} I(\bm{x}_{t + \Delta t})$. Thus, we finish the proof.
\end{proof}

\subsection{ESTIMATION ERROR}
In this section, we analyze the estimation error of FIGD with the MPGD. 
\begin{proposition}
Given a precise energy function $\varepsilon(\bm{\hat{x}}_{0|t},\bm{c})$, the reverse process of the FIGD could be formulated as:
\begin{equation}
\begin{gathered}
    \bm{x}_{t-1} = \hat{m}_{t-1} - \frac{2\rho_{t}}{\sqrt{\hat{a}_{t}}}\nabla_{\bm{\hat{x}}_{0|t}}\varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) \\
    \hat{m}_{t-1} = (1+0.5\beta_{t})\bm{x}_{t} +  \beta_{t}\nabla_{\bm{x}_{t}}\log p(\bm{x}_{t}) + \sqrt{\beta_{t}}\epsilon.
    \label{eq:final sampling}
\end{gathered}
\end{equation}
Assumes $\varepsilon(\bm{\hat{x}}_{0|t},\bm{c})$ following $\kappa$-Lipschitz, we have the upper bound:
\begin{equation}
    ||x^{FIGD}_{t} - x^{MPGD}_{t}||_{2}<  \rho_{t}\kappa(\frac{2\sqrt{\hat{a}_{t-1}}-\sqrt{\hat{a}_{t}}}{\sqrt{\hat{a}_{t}}}).
\end{equation}
\end{proposition}

\begin{proof}
    Based on the $\kappa$-Lipschitz, we first have:
    \begin{equation}
        \nabla_{\bm{\hat{x}}_{0|t}}\varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) < \kappa.
    \end{equation}
Then:
\begin{equation}
\begin{split}
    ||x^{FIGD}_{t} - x^{MPGD}_{t}||_{2} &= \rho_{t} || \frac{2}{\sqrt{\hat{\alpha}_{t}}}\nabla_{\bm{\hat{x}}_{0|t}}\varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) - \sqrt{\hat{a}_{t-1}}\nabla_{\bm{\hat{x}}_{0|t}}\varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) ||_{2}\\
    &\approx \rho_{t}(\frac{2\sqrt{\bm{\hat{a}}_{t-1}}-\sqrt{\bm{\hat{a}}_{t}}}{\sqrt{\bm{\hat{a}}_{t}}})||\nabla_{\bm{\hat{x}}_{0|t}}\varepsilon(\bm{\hat{x}}_{0|t},\bm{c})||_{2} \\
    &<\rho_{t}\kappa(\frac{2\sqrt{\hat{a}_{t-1}}-\sqrt{\hat{a}_{t}}}{\sqrt{\hat{a}_{t}}})
    \label{eq:final sampling}
\end{split}
\end{equation}
Thus, we finish the proof. When $t\rightarrow T$, $\frac{2\sqrt{\hat{a}_{t-1}}-\sqrt{\hat{a}_{t}}}{\sqrt{\hat{a}_{t}}}$ will tend to be large. This further shows the difference between FIGD and MPGD. Meanwhile, when $t\rightarrow 0$,  $\frac{2\sqrt{\hat{a}_{t-1}}-\sqrt{\hat{a}_{t}}}{\sqrt{\hat{a}_{t}}}$ will tend to 0.
\end{proof}


\section{MORE RESULTS}
\begin{figure*}[bt]
    \centering
    \includegraphics[width=\textwidth]{material/supp_style1.pdf}
    \caption{Generation results of training-free style guidance with text-to-image Stable Diffusion. We choose the five styles with different text prompts. It could be found that the generated images well match text prompts and style images. }
    \label{fig:morersutls}
\end{figure*}

\subsection{FACE RELATED TASKS}
\textbf{Text.} Given a pre-trained CLIP, we define that $\mathcal{P}_{\theta_{1}}$ is the vision encoder and $\mathcal{P}_{\theta_{2}}$ is the text encoder, the loss function could be defined as:
\begin{equation}
    \varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) = ||\mathcal{P}_{\theta_{1}}(\bm{\hat{x}}_{0|t})-\mathcal{P}_{\theta_{2}}(\bm{c})||_2,
\end{equation}
where in this task, $\bm{c}$ is the set of text prompts.

\textbf{Parse maps.} Given a pre-trained parse map extractor $\mathcal{P}_{\theta_{_3}}$ that could map the map to the parse map, the loss function could be defined as:
\begin{equation}
    \varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) = ||\mathcal{P}_{\theta_{3}}(\bm{\hat{x}}_{0|t})-\mathcal{P}_{\theta_{3}}(\bm{c})||_2,
\end{equation}
where in this task, $\bm{c}$ is the set of reference images.

\textbf{Sketch.} Given a pre-trained sketch extractor $\mathcal{P}_{\theta_{_4}}$ that could change the image to the related sketch, the loss function could be defined as:
\begin{equation}
    \varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) = ||\mathcal{P}_{\theta_{3}}(\bm{\hat{x}}_{0|t})-\mathcal{P}_{\theta_{3}}(\bm{c})||_2,
\end{equation}
where in this task, $\bm{c}$ is the set of reference images.
\subsection{STABLE DIFFUSION RELATED TASKS}
Given a pre-trained CLIP with the vision encoder $\mathcal{P}_{\theta_{1}}$, the loss function could be defined as:
\begin{equation}
        \varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) = ||G(\mathcal{P}_{\theta_{1}}(\bm{\hat{x}}_{0|t}))-G(\mathcal{P}_{\theta_{1}}(\bm{c}))||_2,
\end{equation}
where $G(\ast)$ is the operation to calculate the Gram matrix and $\bm{c}$ is the set of style reference images.
\subsection{CONTROLNET RELATED TASKS}
\textbf{Face guidance.} Given a pre-trained face detector $\mathcal{P}_{\theta_{5}}$ that could extract the face location with a bounding Box (bbox) and pre-trained parse map extractor $\mathcal{P}_{\theta_{_3}}$, we first extract the bbox of the face and use the $\mathcal{P}_{\theta_{_3}}$ to extract related parse map as the guidance. The loss function could be defined as:
\begin{equation}
            \varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) = ||\mathcal{P}_{\theta_{5}}(\mathcal{P}_{\theta_{3}}(\bm{\hat{x}}_{0|t}))-\mathcal{P}_{\theta_{5}}(\mathcal{P}_{\theta_{3}}(\bm{c}))||_2,
\end{equation}
where $\bm{c}$ is the set of face reference images.

\textbf{Style task.} 
The loss function is the same as the loss function in stable diffusion-related tasks. Given a pre-trained CLIP with the vision encoder $\mathcal{P}_{\theta_{1}}$, the loss function could be defined as:
\begin{equation}
        \varepsilon(\bm{\hat{x}}_{0|t},\bm{c}) = ||G(\mathcal{P}_{\theta_{1}}(\bm{\hat{x}}_{0|t}))-G(\mathcal{P}_{\theta_{1}}(\bm{c}))||_2.
\end{equation}
\section{MORE QUALITATIVE RESULTS}
\subsection{FACE RELATED TASKS}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_2.pdf}
    \caption{Qualitative examples of using a single condition human face images. The included conditions are (a) text, (b) face parsing maps, and (c) sketches. We compare FIGD ($T=50$) with the MPGD ($T=100$), FreeDom ($T=100$), and LGD-MC ($T=100, n=3$). It can be found that MPGD is invalid since these tasks break the linear hypothesis theory, and FIGD performs well.}
    \label{fig:faceresultslgd}
\end{figure*}
\begin{table*}[h!]
    \caption{Quantitative results of face-related tasks. We compare three FreeDom, LGD-MC, and MPGD based on CLIP score for text tasks and FID and distance norms for sketch and parse tasks.}
    \centering
    \begin{tabular}{c c c c c c}
        \toprule
        \multirow{2}{4em}{\textbf{Method}} &  \textbf{Texts} &  \multicolumn{2}{c}{\textbf{Parsing maps}}  & \multicolumn{2}{c}{\textbf{Sketch}} \\
        &\textbf{Distance$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{Distance$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{Distance$\downarrow$}\\
        \midrule
        LGD-MC (T=100, n=3) & 12.90 & 125.50  & 3225.13 & 144.74  & 43.40\\
        FreeDom (T=100)& 10.56 & \textbf{117.77}  & \textbf{2157.22} & 146.43  & 39.94 \\
        MPGD (T=100)& 12.26 & 175.31  &  2837.81 & 154.83  & 28.69 \\
        FIGD (T=100)& \textbf{10.16} & 127.48  &  2224.98 & \textbf{138.80}  & \textbf{27.95}\\
        \bottomrule
    \end{tabular}
\end{table*}
\subsection{STABLE DIFFUSION RELATED TASKS}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_1.pdf}
    \caption{Quantitative results of training-free style guidance with text-to-image Stable Diffusion.}
\end{figure*}

\begin{table*}[h!]
    \caption{Quantitative results of style-guided generation with Stable Diffusion experiment. We compared FIGD with the two baselines, FreeDom and MPGD, in style-guided generation tasks with the Stable Diffusion; we get the overall improvement both in the Style score~\cite{freedom}, CLIP score and the time cost since our method could generate high-quality images with few sampling steps. NA for LGD-MC ($T=100, n=3$) represents that we use shared memory to generate images since the required GPU RAM is over 24GB, and we cannot calculate the precise GPU costs.}
    \centering
    \begin{tabular}{c c c c}
        \toprule
        \textbf{Method} &  \textbf{Style$\downarrow$} &  \textbf{CLIP$\uparrow$} & \textbf{Time(s)} \\
        \midrule
        LGD-MC ($T=100, n=1$) & 254.59 & 30.99 & 63 \\
        LGD-MC ($T=100, n=3$) & 247.39 & 31.28 & NA \\
        FreeDom ($T=100$) & 226.26 & 27.21 & 63 \\
        FreeDom ($T=50$) & 377.96 & \textbf{32.54} & 33 \\ 
        MPGD ($T=100$) & 351.16 & 25.08 & 35 \\
        MPGD ($T=50$) & 408.28 & 23.23 & 18\\
        \midrule
        FIGD ($T=100$)& \textbf{225.83} & 31.87 & 35\\
        FIGD ($T=50$)& 245.51 & 30.84 & 17\\
        FIGD ($T=30$) & 281.67 & 29.07 & \textbf{11}\\
        \bottomrule
    \end{tabular}
\end{table*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_3.pdf}
    \caption{Additional quantitative results of training-free style guidance with text-to-image Stable Diffusion, where we use $T=100$ for FreeDom, MPGD and LGD-MC (n=3) and use $T=50$ for FIGD.}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_4.pdf}
    \caption{Additional quantitative results of training-free style guidance with text-to-image Stable Diffusion, where we use $T=100$ for FreeDom, MPGD and LGD-MC (n=3) and use $T=50$ for FIGD.}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_5.pdf}
    \caption{Additional quantitative results of training-free style guidance with text-to-image Stable Diffusion, where we use $T=100$ for FreeDom, MPGD and LGD-MC (n=3) and use $T=50$ for FIGD.}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_6.pdf}
    \caption{Additional quantitative results of training-free style guidance with text-to-image Stable Diffusion, where we use $T=100$ for FreeDom, MPGD and LGD-MC (n=3) and use $T=50$ for FIGD.}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_7.pdf}
    \caption{Additional quantitative results of training-free style guidance with text-to-image Stable Diffusion, where we use $T=100$ for FreeDom, MPGD and LGD-MC (n=3) and use $T=50$ for FIGD.}
\end{figure*}

\subsection{CONTROLNET RELATED TASKS}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_3.pdf}
    \caption{Qualitative examples of face related tasks based on ControlNet experiments. We compared FIGD ($T=100$) with the FreeDom ($T=100$) and MPGD ($T=100$). }
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_4.pdf}
    \caption{Qualitative examples of style tasks based on ControlNet experiments. We compared FIGD ($T=100$) with the FreeDom ($T=100$) and MPGD ($T=100$). }
    \label{fig:morersutls}
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_5.pdf}
    \caption{Qualitative examples of style tasks based on ControlNet experiments. We compared FIGD ($T=100$) with the FreeDom ($T=100$) and MPGD ($T=100$).}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_1.pdf}
    \caption{QQualitative examples of style tasks based on ControlNet experiments. We compared FIGD ($T=100$) with the FreeDom ($T=100$) and MPGD ($T=100$).}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_2.pdf}
    \caption{Qualitative examples of style tasks based on ControlNet experiments. We compared FIGD ($T=100$) with the FreeDom ($T=100$) and MPGD ($T=100$).}
\end{figure*}

\subsection{Extra Results}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_8.pdf}
    \caption{More qualitative examples of training-free style guidance for FIGD ($T=100$), where the prompt is "a cat wearing glasses".}
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_9.pdf}
    \caption{More qualitative examples of training-free style guidance for FIGD ($T=100$), where the prompt is "a cat wearing glasses".}
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_10.pdf}
    \caption{More qualitative examples of training-free style guidance for FIGD ($T=100$), where the prompt is "a cat wearing glasses".}
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_11.pdf}
    \caption{More qualitative examples of training-free style guidance for FIGD ($T=100$), where the prompt is "a cat wearing glasses".}
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{material/rebuttal_new_12.pdf}
    \caption{More qualitative examples of training-free style guidance for FIGD ($T=100$), where the prompt is "a cat wearing glasses".}
\end{figure*}


